Hands Off my Database: Ransomware Detection in Databases through Dynamic Analysis of Query Sequences

Ransomware is an emerging threat which imposed a \$ 5 billion loss in 2017 and is predicted to hit \$ 11.5 billion in 2019. While initially targeting PC (client) platforms, ransomware recently made the leap to server-side databases - starting in January 2017 with the MongoDB Apocalypse attack, followed by other attack waves targeting a wide range of DB types such as MongoDB, MySQL, ElasticSearch, Cassandra, Hadoop, and CouchDB. While previous research has developed countermeasures against client-side ransomware (e.g., CryptoDrop and ShieldFS), the problem of server-side ransomware has received zero attention so far. In our work, we aim to bridge this gap and present DIMAQS (Dynamic Identification of Malicious Query Sequences), a novel anti-ransomware solution for databases. DIMAQS performs runtime monitoring of incoming queries and pattern matching using Colored Petri Nets (CPNs) for attack detection. Our system design exhibits several novel techniques to enable efficient detection of malicious query sequences globally (i.e., without limiting detection to distinct user connections). Our proof-of-concept implementation targets MySQL servers. The evaluation shows high efficiency with no false positives and no false negatives and very moderate performance overhead of under 5%. We will publish our data sets and implementation allowing the community to reproduce our tests and compare to our results.

==> 06_future_work.tex <==

%\section{Discussion and Future Work}\label{sec:future_work}

%In the previous section, we evaluated the precision of \toolAbrev as well its performance impact.
%To achieve this, we have run multiple experiments. 
%In this section, we will briefly discuss these results and give an outlook future work on this issue. 



%\subsection{Discussion}

%\todoAlexandra{Make it part of evaluation. It is strange to have conclusions about evaluation in a separate section.}
%Results show that \toolAbrev neither creates false-negative nor false-positive classifications for the demonstrated applications. 
%This precision means \toolAbrev will detect every attack that is executed as described.
%At the same time, it will not trigger false alerts leading to unnecessary administrator actions or interfering with regular operations.

%The performance results show that the usage of \toolAbrev only takes about 5\% more resources than without the tool. 
%Thus, \toolAbrev can be used in existing setups with only a small reduction in performance. 
%For larger setups, this would mean an extra server for every 20 servers used.

%Both performance and precision evaluation shows that \toolAbrev is ready to use.
%It increases security without adding false alerts while requiring only few computational resources.
%Since it is a simple MySQL plugin is easily installed and can be readily deployed.

\subsection{Limitation}

%\todoAlexandra{Please move limitations into evaluation and future work into conclusion (no discussion section)}
%For the evaluation of the classification precision, we used the insertion of a BitCoin address to detect the ransom message. \todoAll{This comes out of nowhere, since we never described our policy and never told we detect Bitcoin addresses} 
In future work, we will, on the one hand, have to evaluate whether this is too general and can result in false positives in specific use-cases, e.g., database backends for web forums where a significant amount of BitCoin addresses is exchanged. 
On the other hand for some applications, this might not be generic enough. 
Thus it might be useful to detect for other ways of payments inserted into the ransom message. 
This extension includes other cryptocurrencies as well as PayPal targets and bank account numbers.

The presented results are only for our first ``proof-of-concept implementation.'' 
This implementation is focused on functionality, not speed.
Neither \toolAbrev nor the used Petri net library has been profiled for potential bottlenecks.
Also, no compiler optimization has been enabled.
Thus no general optimization (-Ox) or hardware optimization (-march) regarding the used testbed has been performed.
In future work, we will evaluate this potential to increase performance further. 

Additionally, for the ``modify table'' event this first implementation only checks for ``\texttt{RENAME TABLE}'' statements. 
Future versions can add further capabilities to find other types of modifications, e.g., to detect hidden renames (e.g., moving all content from one table to another).

In this work, we only demonstrate our approach for the use-case of protecting MySQL databases against attacks the described ransom attacks. 
In future work, we plan to address other attack types like using MySQL plugins \todoAlexandra{Sounds wierd. Why using MySQL plugins is an attack?}\todoAll{We plan also to address other attack types like sql injections using mysql LOAD\_FILE() and INTO OUTFILE(); Source: http://blog.rootcon.org/2012/03/sql-injection-using-mysql-loadfile-and.html}
\todoMichael{Query logs for these kind of attacks exist and can also be published.} as well as attacks against other databases like MongoDB.


==> 90_acknowledgments.tex <==
\section*{Acknowledgments}

This work was co-funded by the German Research Foundation (DFG) under grant No. (KO 3445/16-1).

==> figures/approach_process_shrunk.tex <==
%\begin{scaletikzpicturetowidth}{0.48\textwidth}

\tikzset{
  % add this style to all tikzpicture environments
  every picture/.append style={
    % enable scaling of nodes
    transform shape,
    % set scale factor
    scale=0.8
  }
}

\begin{sequencediagram}
    %\newthread{A}{User}{}
    \newthread{B}{Server}{}
    \newinst{C}{Controller}{}
    \newinst{D}{Classifier}{}
    \newinst{E}{Notifier}{}
    \newinst{F}{Rewriter}{}
    %\begin{call}{A}{query}{B}{}
    \begin{call}{B}{alert(1)}{C}{}
        \begin{call}{C}{query(2)}{D}{\begin{tabular}{c}
             classifi- \\
             cation(4)
        \end{tabular}}
            \begin{callself}{D}{evaluate(3)}{} 
            \end{callself}
        \end{call}
        \begin{sdblock}{opt}{classification = malicious} 
            \begin{messcall}{C}{query details(5)}{E}
                \begin{callself}{E}{notify(6)}{} 
                \end{callself}
            \end{messcall}
            \begin{call}{C}{malicious query(7)}{F}{benign query(9)}
                \begin{callself}{F}{rewrite(8)}{} 
                \end{callself}
            \end{call}
        \end{sdblock}
    \end{call}
    \begin{callself}{B}{execute query(10)}{} 
    \end{callself}
    %\end{call}
\end{sequencediagram}
%\end{scaletikzpicturetowidth}

==> tables/classifier_transitions.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{ l | l }
    \hline
    Literal & Transition Actions \\ \hline
    LD & List Databases (e.g. show databases) \\ 
    LT & List Tables \\
    %& e.g. select * from information\_schema.tables \\
    LC & List Columns\\
     %& (e.g. select * from information\_schema.columns) \\
    CT & Create Table (name like `Please Read')\\ 
    DD & Drop Database \\ 
    DT & Drop Table \\ 
    MT & Modify table\\ 
    I & Insert ransom message\\ 
    A & Always \\ \hline
    \end{tabular}
    \caption{Transition Action for the CPN in Figure~\ref{fig:approach_classifierPN}}
    \label{tab:approach_classifierTransitions}
\end{table}
